Finding the Missing-half: Graph Complementary Learning for Homophily-prone and Heterophily-prone Graphs

Real-world graphs generally have only one kind of tendency in their connections. These connections are either homophily-prone or heterophily-prone. While graphs with homophily-prone edges tend to connect nodes with the same class (i.e., intra-class nodes), heterophily-prone edges tend to build relationships between nodes with different classes (i.e., inter-class nodes). Existing GNNs only take the original graph during training. The problem with this approach is that it forgets to take into consideration the ``missing-half" structural information, that is, heterophily-prone topology for homophily-prone graphs and homophily-prone topology for heterophily-prone graphs. In our paper, we introduce Graph cOmplementAry Learning, namely GOAL, which consists of two components: graph complementation and complemented graph convolution. The first component finds the missing-half structural information for a given graph to complement it. The complemented graph has two sets of graphs including both homophily- and heterophily-prone topology. In the latter component, to handle complemented graphs, we design a new graph convolution from the perspective of optimisation. The experiment results show that GOAL consistently outperforms all baselines in eight real-world datasets.

==> sections/explore.tex <==
To build effective graph convolution for complemented graphs, we first need to explore the effect of different types of spectral filters including low-pass, high-pass, band-pass, and band-rejection filters. This analysis guides us to select and design filters for different types of topology. 

Specifically, we provide a general pipeline to analyse spectral filters. Firstly, we derive the graph convolution form given a specific spectral filter function as shown in \ref{sec: bridging}. Based on the derived convolution, we infer its optimisation form to understand how the spectral filter works. In addition, with the optimisation form, we can deduce what kind of topology is desired for the specific spectral filter. We present in Appendix \textbf{X} the analysis results for different spectral filters in terms of their graph convolution and objective form.

\textbf{insert a table including columns: name of spectral filters/function form/propagation form/objective form}

\textbf{insert a figure drawing all different kinds of filters}

\subsection{Low-pass Filter}

\textbf{Effect.} Existing GNN approaches primarily use low-pass filters, e.g., GCN, SGC, and APPNP~\cite{he2021bernnet}. Here, we analyse a typical linear low-pass filter:
\begin{equation}
    \textbf{F}_{low}(\lambda) = 1 - \lambda,
    \label{eq:filter low}
\end{equation}
% where $\alpha \in {(0,1)}$ is a parameter that controls the slope of the linear filter function. We set $\alpha$ in this range so that at least half of the lower spectrum can be retained when $\alpha$ approaches 1. Conversely, when $\alpha$ becomes 0, the low-pass effect degrades as the function slope become flatter. 
Based on Equation~\ref{eq:gconv kernel} and Equation~\ref{eq:message passing form}, we can infer its graph convolution form is:
\begin{align}
    \begin{aligned}
            \mathcal{A} &=  \hat{\textbf{A}},
        \\ \textbf{H}^{l + 1}  &= \sigma(\hat{\textbf{A}}\textbf{H}^{l}\textbf{W}^{l}).
\end{aligned}
\label{eq:gconv low}
\end{align}

\begin{proposition}
For the defined linear low-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\begin{equation}
\normalfont{
    \mathcal{O}_{low} = \underset{\textbf{H}}{min}\{
tr(\textbf{H}^T\hat{\textbf{L}}\textbf{H})\} = \frac{1}{2} \sum^E_{(i,j) \in \mathcal{E}} \hat{\textbf{A}}_{i,j} \parallel\textbf{H}_i-\textbf{H}_j\parallel^2},
    \label{eq:low obj}
\end{equation}
\end{proposition}
\begin{proof}
This objective can be solved with $\frac{\partial  tr(\textbf{H}^T\hat{\textbf{L}}\textbf{H})}{\partial \textbf{H}} = 0$ as the objective is a convex function. This is because $\hat{\textbf{L}}$ is a positive semi-definite matrix. Thus, we can derive:
\begin{align}
\begin{aligned}
\hat{\textbf{L}}\textbf{H} = 0 &\to  \textbf{H} -  \hat{\textbf{A}}\textbf{H} = 0  \to \textbf{H} = \hat{\textbf{A}}\textbf{H}
% \\ &\to \textbf{H} - \hat{\textbf{A}}\textbf{H} = 0 \\ &\to \textbf{H} = ((1 - \alpha)\textbf{I} + \alpha \hat{\textbf{A}})\textbf{H}
\end{aligned}
\end{align}
Here, we can see the derived formula is consistent with the inferred graph convolution form. This result is also validated in ~\cite{zhu2021interpreting}. Thus, we prove the proposition. 

\end{proof}

\textbf{Desired Topology.}
From Equation~\ref{eq:low obj}, it is evident that the linear low-pass filter minimises the Euclidean distance between two connected nodes. This indicates the filtering process relies heavily on the homophilic-prone edges of a given graph. When homophilic-prone edges are dominant in a graph, same-class nodes can be clustered using low-pass filters. In contrast, if a graph is highly heterophilic-prone, these low-pass filters tend to maximise the similarity between inter-class nodes and lead to poor performance. This explains why low-pass-based GNNs such as GCN~\cite{kipf2016semi} and GAT~\cite{velivckovic2017graph} work poorly on heterophilic graphs. Thus, the desired topology for low-pass filters is homophilic-prone graphs.

\subsection{High-pass Filter}
\textbf{Effect.} Some existing works incorporate linear high-pass filters to capture information for the high-frequency band of graph signals \cite{fagcn2021,wu2022beyond}. Here, we explore the following linear high-pass filter:
\begin{equation}
    \textbf{F}_{high}(\lambda) = \lambda \hlt{-1},
\label{eq:filter high}
\end{equation}
% where $\alpha \in {(0,1)}$ is still used to adjust the function slope. 
% In contrast to Equation~\ref{eq:filter low}, here, when $\alpha$ close to 1, it retained the half of the higher spectrum. 
The graph convolution form of Equation~\ref{eq:filter high} can be defined as:
\begin{align}
    \begin{aligned}
        \mathcal{A} &=  - \hat{\textbf{A}}, \\
        \textbf{H}^{l + 1} &= \sigma(-\hat{\textbf{A}}\textbf{H}^l\textbf{W}^l),
    \end{aligned}
        \label{eq:gconv high}
\end{align}
\begin{proposition}
For the defined linear high-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\end{proposition}
\vspace{-5mm}
\begin{align}
    \begin{aligned}
    \mathcal{O}_{high} &= \underset{\textbf{H}}{min}\{
    tr(\textbf{H}^T(\textbf{I} +  \hat{\textbf{A}})\textbf{H})\}\\ 
    \end{aligned}
    \label{eq:high obj}
\end{align}

\begin{proof}
    Here, we make an assumption that $\hat{\textbf{A}}$ is connected and non-bipartite. As such, $\hat{\textbf{A}}$ would be positive semi-definite and
    % As $\hat{\textbf{A}}$ and $\textbf{I}$ are all positive definite matrices, 
    the objective is still a convex function. Thus, it can be solved via $\frac{\partial tr(\textbf{H}^T(\textbf{I} + \hat{\textbf{A}})\textbf{H})}{\partial \textbf{H}} = 0$:
\begin{align}
    \begin{aligned}
    (\textbf{I} + \hat{\textbf{A}})\textbf{H} = 0  &\to \textbf{H} = -\hat{\textbf{A}}\textbf{H}.
    \end{aligned}
\end{align}
As the derived equation is consistent with Equation~\ref{eq:gconv high} without learnable parameters and non-linearity, we prove the proposition.
\end{proof}
We can easily observe that Objective~\ref{eq:high obj} is minimising the dot product similarity between each dimension of graph representation $\textbf{H} \in \mathbb{R}^{N \times D'}$ and the convoluted representation
$(\textbf{I} + \hat{\textbf{A}})\textbf{H}$:
\begin{align}
    \begin{aligned}
        \mathcal{O}_{high} &= \underset{\textbf{H}}{min}\{
    tr(\textbf{H}^T(\textbf{I} + \hat{\textbf{A}})\textbf{H}), \\ &= \sum^{D'}_k\textbf{H}^T_k(((\textbf{I} + \hat{\textbf{A}})\textbf{H})[{:,k}]),
    \end{aligned}
    \label{eq:high obj simple}
\end{align}

\textbf{Desired Topology.} Equation~\ref{eq:high obj simple} indicates that the desired topology for linear high-pass filters should be heterophilic-prone graphs. Here, we consider $\hat{\textbf{H}} = (\textbf{I} + \hat{\textbf{A}})\textbf{H}$. If $\hat{\textbf{A}}$ is a homophilic-prone graph, the convoluted representation can be regarded as a subgraph-level embedding encapsulating mainly 1-hop intra-class neighbouring information. Thus, the dot product similarity between $\textbf{H}$ and $\hat{\textbf{H}}$ (serving as a positive sample) should be maximised instead of minimised in this case. In contrast, $\hat{\textbf{A}}$ generated with heterophilic-prone graphs aggregating inter-class neighbours and thus $\hat{\textbf{H}}$ can be considered as negative samples. In this case, minimising the dot product similarity between ${\textbf{H}}$ and $\hat{\textbf{H}}$ is reasonable.
 
\subsection{Band-pass Filter}
\textbf{Effect.} Band-pass filters bulged the middle component of frequency bands in graph signals. Since linear functions are incapable of suppressing both low and high-frequency bands, we use a quadratic form instead to achieve this:
\begin{equation} 
    \textbf{F}_{band}(\lambda) = -(\lambda - 1)^2 + 1,      
    \label{eq:filter band}
\end{equation}
Following the same practice as the aforementioned two filters, the graph convolution form of Equation~\ref{eq:filter band} is:
\begin{align}
    \begin{aligned}
        \mathcal{A} &= \textbf{I} - \hat{\textbf{A}}^2, \\
        \textbf{H}^{l + 1}  &= \sigma((\textbf{I} - \hat{\textbf{A}}^2)\textbf{H}^{l}\textbf{W}^{l}).
    \end{aligned}
\end{align}
\begin{proposition}
For the defined band-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\end{proposition}
\vspace{-5mm}
\begin{align}
    \begin{aligned}
    \mathcal{O}_{band} &= \underset{\textbf{H}}{min}\{
     tr(\textbf{H}^T \hat{\textbf{A}}^2\textbf{H})\},\\ &= \sum^{D'}_k\textbf{H}^T_k(( \hat{\textbf{A}}^2\textbf{H})[{:,k}]).
    \end{aligned} 
    \label{eq:band obj}
\end{align}
\begin{proof}
    Here, we still have the assumption that $\hat{\textbf{A}}$ is connected and non-bipartite. As the product of positive semi-definite matrices is still positive definite iff the product is symmetric, we can deduce the objective Equation~\ref{eq:band obj} is still a convex function~\cite{meenakshi1999product}. As such, we can solve this objective by setting $\frac{\partial tr(\textbf{H}\hat{\textbf{A}}^2\textbf{H})}{\partial \textbf{H}} = 0$:
    \begin{align}
        \begin{aligned}
        \hat{\textbf{A}}^2\textbf{H} = 0 &\to \hlt{\textbf{H} \hat{\textbf{A}}^2 \textbf{H} = \textbf{H}}\\ &\to \textbf{H} = (\textbf{I} -  \hat{\textbf{A}}^2)\textbf{H} 
        \end{aligned}
    \end{align}
    Here, we prove the proposition above.
\end{proof}

\textbf{Desired Topology.} From Equation~\ref{eq:band obj}, we can see this objective is similar to Equation~\ref{eq:high obj simple}, the linear high-pass filters. The main difference between these two equations is Equation~\ref{eq:band obj} takes the second-hop neighbourhood into account when conducting aggregation. Thus, the desired topology for the \hlt{defined band-pass filter is still heterophilic-prone graphs.} The $i,j$ entry of $n$-th power of $\hat{\textbf{A}}$ represents the probability of a random walk starting from node $i$ and ending up at node $j$ after $n$ steps.  


% \subsection{Band-reject Filter}
% \textbf{Effect.} In contrast to band-pass filters, band-reject filters constrain the middle-frequency band of graph signals. Thus, we also use a quadratic form to achieve this:
% \begin{equation}
%     \textbf{F}_{mid}(\lambda) = (\lambda - 1)^2,
%     \label{eq:filter band_rej}
% \end{equation}
% % where $\alpha > 0$ and it is smaller, the function focuses more on low and high frequency signals. 
% Its graph convolution form can be defined as:
% \begin{align}
%     \begin{aligned}
%         \mathcal{A} &= \hat{\textbf{A}}^2, \\
%         \textbf{H}^{l + 1}  &= \sigma( \hat{\textbf{A}}^2\textbf{H}^{l}\textbf{W}^{l}).
%     \end{aligned}
% \end{align}
% \begin{proposition}
% For the defined band-reject filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
% \label{pro: bandrej}
% \end{proposition}
% \vspace{-5mm}
% \begin{align}
%     \begin{aligned}
%     \mathcal{O}_{bandrej} &= \underset{\textbf{H}}{min}\{
%      tr(\textbf{H}^T (\textbf{I} - \hat{\textbf{A}}^2)\textbf{H})\}, \\ &= \frac{1}{2} \sum^{E'}_{(i,j) \in \mathcal{E'}}\hat{\textbf{A}}^2_{i,j} \parallel \textbf{H}_i - \textbf{H}_j \parallel^2,
%     \end{aligned} 
%     \label{eq:bandrej obj}
% \end{align}
% where $E'$ and $\mathcal{E}'$ are the number of edges and the edge set of $\hat{\textbf{A}}^2$, respectively. 
% \begin{proof}
% From Equation~\ref{eq:bandrej obj}, we can see it is a least square regression objective, which is a convex optimisation problem. Therefore, when $        \frac{\partial \textbf{H}^T(\textbf{I}- \hat{\textbf{A}}^2)\textbf{H}}{\partial \textbf{H}} = 0$:
% \begin{equation}
%     (\textbf{I}-\hat{\textbf{A}}^2)\textbf{H} = 0 \to \textbf{H} = \hat{\textbf{A}}^2\textbf{H}
% \end{equation}
% Thus, we prove Proposition~\ref{pro: bandrej}.
% \end{proof}

% \textbf{\hlt{Desired Topology}.} Similar to low-pass filters objective Equation~\ref{eq:low obj}, the defined band-reject filter is conducting Euclidean distance minimisation between connected nodes. The only difference here is the connection of $\hat{\textbf{A}}^2$ including second-hop neighbours and thus is denser than $\hat{\textbf{A}}$. 

\subsection{Overall Analysis}
To validate that the induced desired topology is consistent with corresponding filters, we conduct experiments using synthetic datasets, and the result is presented in Appendix~\ref{sec:appendix compare filters}.

In summary, the linear low-pass filter and band-reject filter we analysed are suitable for processing homophilic-prone graphs, whereas the linear high-pass filter and the band-pass filter can effectively process heterophilic-prone graphs.

==> sections/explore_backup.tex <==
In this section, we explore the effect of different types of spectral filters including low-pass, high-pass, band-pass, and band-rejection filters. Specifically, we provide a general pipeline to analyse spectral filters. Firstly, we derive the graph convolution form given a specific spectral function. Based on the derived convolution, we infer its optimisation form to understand how the spectral filter works. In addition, with the optimisation form, we can deduce what kind of graph input (i.e., graph structure) is desired for the specific spectral filter.

\textbf{insert a table including columns: name of spectral filters/function form/propagation form/objective form}

\textbf{insert a figure drawing all different kinds of filters}

\subsection{Low-pass Filters}

\textbf{Effect.} Existing GNN approaches primarily use low-pass filters, e.g., GCN, SGC, and APPNP~\cite{he2021bernnet}. We define linear low-pass filters as:
\begin{equation}
    \textbf{F}_{low}(\lambda) = 1 - \lambda,
    \label{eq:filter low}
\end{equation}
where $\alpha \in {(0,1)}$ is a parameter that controls the slope of the linear filter function. We set $\alpha$ in this range so that at least half of the lower spectrum can be retained when $\alpha$ approaches 1. Conversely, when $\alpha$ becomes 0, the low-pass effect degrades as the function slope become flatter. Based on Equation~\ref{eq:gconv kernel} and Equation~\ref{eq:message passing form}, we can infer its graph convolution form is:
\begin{align}
    \begin{aligned}
            \mathcal{A} &=  (1 - \alpha)\textbf{I} + \alpha\hat{\textbf{A}},
        \\ \textbf{H}^{l + 1}  &= \sigma(((1 - \alpha)\textbf{I} + \alpha\hat{\textbf{A}})\textbf{H}^{l}\textbf{W}^{l}).
\end{aligned}
\label{eq:gconv low}
\end{align}

\begin{proposition}
For the defined linear low-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\begin{equation}
\normalfont{
    \mathcal{O}_{low} = \underset{\textbf{H}}{min}\{
    \alpha tr(\textbf{H}^T\hat{\textbf{L}}\textbf{H})\} = \frac{\alpha}{2} \sum^E_{(i,j) \in \mathcal{E}} \hat{\textbf{A}}_{i,j} \parallel\textbf{H}_i-\textbf{H}_j\parallel^2},
    \label{eq:low obj}
\end{equation}
\end{proposition}
\begin{proof}
This objective can be solved with $\frac{\partial \alpha tr(\textbf{H}^T\hat{\textbf{L}}\textbf{H})}{\partial \textbf{H}} = 0$ as the objective is a convex function. This is because $\hat{\textbf{L}}$ is a positive semi-definite matrix. Thus, we can derive:
\begin{align}
\begin{aligned}
\alpha \hat{\textbf{L}}\textbf{H} = 0 &\to \alpha \textbf{H} - \alpha \hat{\textbf{A}}\textbf{H} = 0 
\\ &\to \textbf{H} - (1 - \alpha)\textbf{H} - \alpha \hat{\textbf{A}}\textbf{H} = 0 \\ &\to \textbf{H} = ((1 - \alpha)\textbf{I} + \alpha \hat{\textbf{A}})\textbf{H}
\end{aligned}
\end{align}
Here, we can see the derived formula is consistent with the inferred graph convolution form. Thus, we prove the proposition. 

\end{proof}

\textbf{Desired Graph Input.}
From Equation~\ref{eq:low obj}, it is evident that the linear low-pass filter minimises the Euclidean distance between two connected nodes. This indicates the filtering process relies heavily on the homophily of a given graph. When homophily is high, same-class nodes can be clustered using low-pass filters. In contrast, if a graph is highly heterophilic, these low-pass filters tend to maximise similarity between inter-class nodes and lead to poor performance. This explains why low-pass-based GNNs such as GCN~\cite{kipf2016semi} and GAT~\cite{velivckovic2017graph} work poorly on heterophilic graphs. Thus, the desired graph input for low-pass filters are homophilic graphs.

\subsection{High-pass Filters}
\textbf{Effect.} Some existing works incorporate linear high-pass filters to capture information for the high frequency band of graph signals \cite{fagcn2021,wu2022beyond}. Here, we explore linear high-pass filters:
\begin{equation}
    \textbf{F}_{high}(\lambda) = \alpha \lambda - 1,
\label{eq:filter high}
\end{equation}
where $\alpha \in {(0,1)}$ is still used to adjust the function slope. In contrast to Equation~\ref{eq:filter low}, here, when $\alpha$ close to 1, it retained the half of the higher spectrum. The graph convolution form of~\ref{eq:filter high} can be defined as:
\begin{align}
    \begin{aligned}
        \mathcal{A} &= (\alpha - 1)\textbf{I} - \alpha \hat{\textbf{A}}, \\
        \textbf{H}^{l + 1} &= \sigma(((\alpha - 1)\textbf{I} - \alpha\hat{\textbf{A}})\textbf{H}^l\textbf{W}^l),
    \end{aligned}
        \label{eq:gconv high}
\end{align}
\begin{proposition}
For the defined linear high-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\end{proposition}
\vspace{-5mm}
\begin{align}
    \begin{aligned}
    \mathcal{O}_{high} &= \underset{\textbf{H}}{min}\{
    tr(\textbf{H}^T((2 - \alpha)\textbf{I} + \alpha \hat{\textbf{A}})\textbf{H})\}\\ 
    \end{aligned}
    \label{eq:high obj}
\end{align}

\begin{proof}
    As $\hat{\textbf{A}}$ and $\textbf{I}$ are all positive definite matrices, the objective is still a convex function. Thus, it can be solved via $\frac{\partial tr(\textbf{H}^T((2 - \alpha)\textbf{I} + \alpha \hat{\textbf{A}})\textbf{H})}{\partial \textbf{H}} = 0$:
\begin{align}
    \begin{aligned}
    ((2 - \alpha)\textbf{I} + \alpha \hat{\textbf{A}})\textbf{H} = 0 &\to ((\alpha - 2)\textbf{I} - \alpha \hat{\textbf{A}})\textbf{H} = 0 \\ &\to \textbf{H} = ((\alpha - 1)\textbf{I} - \alpha \hat{\textbf{A}})\textbf{H}
    \end{aligned}
\end{align}
As the derived equation is identical to Equation~\ref{eq:gconv high} without learnable parameters and non-linearity, we prove the proposition.
\end{proof}
In Equation~\ref{eq:high obj}, we can consider $\alpha$ as a weighting term to determine the contribution of $\textbf{I}$ and $\hat{\textbf{A}}$ in the summation $\textbf{I} + \hat{\textbf{A}}$. For simplicity, we set $\alpha = 1$ to let them contribute equally. Then, we can easily observe that this objective is minimising the dot product similarity between each dimension of graph representation $\textbf{H} \in \mathbb{R}^{N \times D'}$ and convoluted representation
$(\textbf{I} + \hat{\textbf{A}})\textbf{H}$:
\begin{align}
    \begin{aligned}
        \mathcal{O}_{high} &= \underset{\textbf{H}}{min}\{
    tr(\textbf{H}^T(\textbf{I} + \hat{\textbf{A}})\textbf{H}), \\ &= \sum^{D'}_k\textbf{H}^T_k(((\textbf{I} + \hat{\textbf{A}})\textbf{H})[{:,k}]),
    \end{aligned}
    \label{eq:high obj simple}
\end{align}

\textbf{Desired Graph Input.} Equation~\ref{eq:high obj simple} indicates that the desired graph input for linear high-pass filters should be heterophilic graphs. Here, we consider $\hat{\textbf{H}} = (\textbf{I} + \hat{\textbf{A}})\textbf{H}$. If $\hat{\textbf{A}}$ is homophilic graphs, the convoluted representation can be regarded as a subgraph-level embedding encapsulating 1-hop homophilic neighbouring information. Thus, the dot product similarity between $\textbf{H}$ and $\hat{\textbf{H}}$ (serving as positive sample) should be maximised instead of minimised in this case. In contrast, $\hat{\textbf{A}})$ generated with heterophilic graphs aggregating inter-class neighbours and thus can be considered as negative sample, which makes the objective Equation~\ref{eq:high obj simple} reasonable.
 
\subsection{Band-pass Filters}
\textbf{Effect.} Band-pass filters bulged the middle component of frequency bands in graph signals. Since linear functions are incapable of suppressing both low and high frequency bands, we use a quadratic form instead to achieve this:
\begin{equation}
    \textbf{F}_{band}(\lambda) = -\alpha(\lambda - 1)^2 + 1,
    \label{eq:filter band}
\end{equation}
where $\alpha > 0$ can shrink or stretch the quadratic function. When $\alpha$ is larger, the suppression on both low and high frequency signals is harder. Following same practice as the aforementioned two filters, the graph convolution form of Equation~\ref{eq:filter band} is:
\begin{align}
    \begin{aligned}
        \mathcal{A} &= \textbf{I} - \alpha \hat{\textbf{A}}^2, \\
        \textbf{H}^{l + 1}  &= \sigma((\textbf{I} - \alpha \hat{\textbf{A}}^2)\textbf{H}^{l}\textbf{W}^{l}).
    \end{aligned}
\end{align}
\begin{proposition}
For the defined band-pass filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\end{proposition}
\vspace{-5mm}
\begin{align}
    \begin{aligned}
    \mathcal{O}_{band} &= \underset{\textbf{H}}{min}\{
    \alpha tr(\textbf{H}^T \hat{\textbf{A}}^2\textbf{H})\},\\ &= \alpha\sum^{D'}_k\textbf{H}^T_k(( \hat{\textbf{A}}^2\textbf{H})[{:,k}]).
    \end{aligned} 
    \label{eq:band obj}
\end{align}
\begin{proof}
    As the product of positive definite matrices are still positive definite iff the product is symmetric, we can deduce the objective Equation~\ref{eq:band obj} is still a convex function~\cite{meenakshi1999product}. As such, we can solve this objective by setting $\frac{\partial tr(\textbf{H}\hat{\textbf{A}}^2\textbf{H})}{\partial \textbf{H}} = 0$:
    \begin{align}
        \begin{aligned}
            \alpha\hat{\textbf{A}}^2\textbf{H} = 0 &\to \textbf{H} -\alpha \hat{\textbf{A}}^2 \textbf{H} = \textbf{H}\\ &\to \textbf{H} = (1 - \alpha \hat{\textbf{A}}^2)\textbf{H} 
        \end{aligned}
    \end{align}
    Here, we prove the proposition above.
\end{proof}

\textbf{Desired Graph Input.} From Equation~\ref{eq:band obj}, we can see this objective is similar to Equation~\ref{eq:high obj simple}, the linear high-pass filters. The main difference between these two equations is Equation~\ref{eq:band obj} takes the second-hop neighbourhood into account when conducting aggregation. Thus, the desired graph input for the defined band-pass filter is still homophilic graphs.  


\subsection{Band-reject Filters}
\textbf{Effect.} In contrast to band-pass filters, band-reject filters constrain the middle frequency band of graph signals. Thus, we also use a quadratic form to achieve this:
\begin{equation}
    \textbf{F}_{mid}(\lambda) = \alpha(\lambda - 1)^2,
    \label{eq:filter band_rej}
\end{equation}
where $\alpha > 0$ and it is smaller, the function focuses more on low and high frequency signals. Its graph convolution form can be defined as:
\begin{align}
    \begin{aligned}
        \mathcal{A} &= \alpha \hat{\textbf{A}}^2, \\
        \textbf{H}^{l + 1}  &= \sigma( \alpha\hat{\textbf{A}}^2\textbf{H}^{l}\textbf{W}^{l}).
    \end{aligned}
\end{align}
\begin{proposition}
For the defined band-reject filter, ignoring the effect of $\textbf{W}^{l}$ and the non-linearity $\sigma(\cdot)$ in each layer, its optimisation objective is:
\label{pro: bandrej}
\end{proposition}
\vspace{-5mm}
\begin{align}
    \begin{aligned}
    \mathcal{O}_{bandrej} &= \underset{\textbf{H}}{min}\{
     tr(\textbf{H}^T (\textbf{I} - \alpha\hat{\textbf{A}}^2)\textbf{H})\}, \\ &= \frac{\alpha}{2} \sum^{E'}_{(i,j) \in \mathcal{E'}}\hat{\textbf{A}}^2_{i,j} \parallel \textbf{H}_i - \textbf{H}_j \parallel^2,
    \end{aligned} 
    \label{eq:bandrej obj}
\end{align}
where $E'$ and $\mathcal{E}'$ are the number of edges and the edge set of $\hat{\textbf{A}}^2$, respectively. 
\begin{proof}
From Equation~\ref{eq:bandrej obj}, we can see it is a least square regression objective, which is a convex optimisation problem. Therefore, when $        \frac{\partial \textbf{H}^T(1-\alpha \hat{\textbf{A}}^2)\textbf{H}}{\partial \textbf{H}} = 0$:
\begin{equation}
    (1-\alpha \hat{\textbf{A}}^2)\textbf{H} = 0 \to \textbf{H} = \alpha \hat{\textbf{A}}^2\textbf{H}
\end{equation}
Thus, we prove Proposition~\ref{pro: bandrej}.
\end{proof}

\textbf{Desired Graph Input.} Similar to low-pass filters objective Equation~\ref{eq:low obj}, the defined band-reject filter is conducting Euclidean distance minimisation between connected nodes. The only difference here is the connection of $\hat{\textbf{A}}^2$ including second-hop neighbours and thus is denser than $\hat{\textbf{A}}$. The $i,j$ entry of $n-th$ power of $\hat{\textbf{A}}$ represents the probability of a random walk starting from node $i$ and end up at node $j$ after $n$ steps.

\subsection{Overall Analysis}
Based on the aforementioned analysis of various spectral filters, we can observe that 

==> sections/method_gcl_bakcup.tex <==
In this section, we introduce graph complementary learning, which includes two main steps: graph discrimination and graph complementation. Graph discrimination is used to determine  what kind of structural information is missing from a graph. The latter step aims to find the missing-half structural information to complement the graph. The pipeline of graph complementary learning is illustrated in Figure~\ref{fig:overall} (a).

% The first component is designed to complement the original graph with an additional type of structural information, while the latter is designed to handle graphs encoding both homophilic-prone and heterophilic-prone structural information.

% \subsection{Graph Complementary Learning}
% Graph complementary learning has two main steps including graph discrimination and graph complementation.

\subsection{Graph Discrimination}
The first step is to determine which type of structural information is missing from a graph. As an example, the Cora graph requires heterophilic-prone edges to be complemented, as its edges are homophilic-prone. 

 Given a node pair $(v_i, v_j)$ The cosine similarity  can be calculated as follows:
 \begin{equation}
     cos(v_i, v_j) = \frac{dot(x_i,x_j)}{\parallel x_i \parallel \parallel x_j \parallel},
 \end{equation}
 where $cos(\cdot)$ takes a node pair as input and outputs the cosine similarity between the two nodes. $dot(\cdot)$ is the dot product similarity between two nodes. $x_i \in \mathbb{R}^{1 \times D}$ is the raw feature for node $i$, and $\parallel x_i \parallel$ means the norm of $x_i$.

We observe that, in homophilic-prone graphs, the \hlt{cosine similarity distribution (CSD) of connected node pairs (i.e., $\{cos(v_i, v_j)|(v_i, v_j) \in \mathcal{E}$\})}
differs greatly from that of randomly sampled node pairs.

In contrast, CSDs in heterophilic-prone graphs are normally close to those in randomly sampled node pairs. To illustrate this observation, we compare the CSD between connected and randomly sampled node pairs for eight datasets in Figure~\ref{fig:cosine comp}. This figure shows that CSDs of connected nodes are normally right-shifted and flatter than those of sampled node pairs in homophilic-prone graphs, while heterophilic-prone graphs remain nearly the same distribution. The right-shiftiness is reasonable as homophilic-prone linkages tend to connect intra-class nodes which have a higher similarity. In addition, homophilic-prone graphs exclude many inter-class node pairs with low similarity, which causes the distribution to be flatter. 

On the other hand, heterophilic-prone graphs have similar distributions to sampled node pairs. The reason for this, we suggest, is that randomly sampled pairs of nodes tend to have mainly heterophilic relationships. \hlt{As shown in Figure~\ref{fig:cosine comp}, the CSDs of randomly sampled pairs across all datasets are heavily right-skewed, which means most sampled pairs have very low cosine similarity}.

% since datasets tend to have low cosine similarity between node pairs. 



% We provide further analysis for this phenomenon in Appendix \textbf{X}.

% This is reasonable as homophilic-prone linkages tend to connect intra-class nodes which are similar while avoiding connecting inter-class nodes that are dissimilar. Heterophilic connections have similar distributions to all node pairs, as the inter-class relationship is dominant across all node pairs.

We propose Kolmogorov-Smirnov statistics (K-S statistics)~\cite{lilliefors1967kolmogorov} to evaluate the difference in distribution between connected and sampled node pairs to determine which kind of connection is likely missing. A desirable property of this measure is that it ranges from 0 to 1, which allows fair comparison between different datasets. K-S statistics can be calculated with the following formula:
\begin{equation}
    KS(\textbf{d}_1, \textbf{d}_2) = max \parallel F(\textbf{d}_1) - F(\textbf{d}_2) \parallel,
\end{equation}
where $KS(\cdot)$ takes two distributions as input and output K-S statistics. $F(\cdot)$ is a function to calculate the cumulative distribution function (CDF) of the given distribution. $F(\textbf{d}_1)$ is the sample CDF and $F(\textbf{d}_2)$ is the reference CDF. In our case, $\textbf{d}_1$ and $\textbf{d}_2$ are the CSDs of connected nodes and randomly sampled nodes, respectively.

If the K-S statistics of a graph exceed 0.2, it will be considered homophilic-prone, otherwise, it will be considered heterophilic-prone. The threshold value of 0.2 is chosen as it indicates a clear/distinguishable difference between two distributions as suggested in \cite{da2021survey}. For each dataset, we randomly sampled ten sets of random node pairs and calculate K-S statistics between these sets and the CSD of connected nodes. The result are averaged and shown in Figure~\ref{fig:cosine comp}. From the figure, we can see this approach successfully distinguishes all graphs (i.e., Cora, CiteSeer, PubMed, Computers and Photo are homophilic-prone / Chameleon, Squirrel, and Actor are heterophilic-prone).

\begin{figure*}
    \centering
\includegraphics[scale = 0.37]{figures/NG_architecture.pdf}
    \caption{The architecture of new graph convolution network. Firstly, we perform graph discrimination to determine which parts of structural information are missing from the input graph. Then, We conduct graph completion to complement the input graph. This process utilises two losses including grouping loss and learning-to-rank loss. While the first loss aim to cluster intra-class nodes, the latter one attempts to predict the correct ranking of neighbour nodes for a target node (e.g., node a in the figure). Graph convolution layers use the complemented graph as input. There are both heterophilic-prone and homophilic-prone connections involved in the convolution at every node. Here, the dotted line and solid line indicate two different types of connections. Grey neighbouring nodes with a white centre point are involved in the convolution process. Finally, we obtain the output prediction for each node, e.g., red-coloured nodes for A class and blue-coloured nodes for B class.}
    \label{fig:overall}
\end{figure*}

\subsection{Graph Complementation}
In this process, we aim to complement the given graph with additional structural information. 

\paragraph{Grouping Loss.} Firstly, we obtain node embeddings with a backbone GNN encoder, e.g., GAT. Then, node embeddings are input to a (Multi-layer Perceptron) MLP model to conduct two tasks: nodes grouping and learning to rank. The first task aims to group intra-class nodes while separating inter-class nodes. Specifically, we first obtain all intra-class node pairs as the positive pairs set $\mathbb{P} = \{(v_i, v_j) | Y_{v_i} = Y_{v_j}\}$, while all inter-class node pairs as the negative set $\mathbb{N} = \{(v_i, v_j) | Y_{v_i} \neq Y_{v_j}\}$. Here $v_i$ and $Y_i$ represent node $i$ and its class, respectively. Then, we calculate the grouping loss to evaluate the grouping correctness. The whole process can be formulated as follows:
\begin{equation}
        \rm \textbf{Z}_{gc} = MLP(\textbf{Z}_{gnn}); \textbf{Z}_{gnn}  = GNN(\mathcal{G}),
\end{equation}
\begin{equation}
    \mathcal{L}_{pos} = - log (\sigma(\frac{\sum_{(i,j) \in \mathbb{P}}\textbf{Z}_{gc}^T[v_i] \cdot \textbf{Z}_{gc}[v_j]}{|\mathbb{P}|}) + \epsilon),
\end{equation}
\begin{equation}
     \mathcal{L}_{neg} = -log (1 - \sigma(\frac{\sum_{(i,j)\in \mathbb{N}}\textbf{Z}_{gc}^T[v_i] \cdot \textbf{Z}_{gc}[v_j]}{|\mathbb{N}|} + \epsilon)),
\end{equation}
 \begin{equation}
         \mathcal{L}_{grp} = \mathcal{L}_{pos} + \mathcal{L}_{neg},
         \label{eq:group loss}
 \end{equation}
 where $\cdot$ represents matrix multiplication, $\textbf{Z}_{gnn}$ is the output embedding of the GNN encoder taking $\mathcal{G}$ as input, 
, $\textbf{Z}_{gc}$ is the output embedding of the MLP model, $\sigma(\cdot)$ is the sigmoid function, $\epsilon$ is a tiny number to prevent computation error. Note that $\textbf{Z}_{gnn}$ is obtained by the \hlt{supervised trained GNN encoder with cross-entropy loss}. We take the output embedding before the prediction layer as $\textbf{Z}_{gnn}$.

\paragraph{Learning-to-Rank Loss.} We adopt ListNet loss ~\cite{cao2007learning}, a learning-to-rank approach, to conduct the second task. It can optimise the ranking of a list of items by minimising the cross entropy between the predicted and true ranking of items. To compute the ranking list $R_i$ for a target node $i$, we first sort its intra-class nodes based on cosine similarity and obtain $L^{intra}_{i} = \{v^{1}_j, ... v^{t}_j| Y_{v^{t}_j} = Y_i ; cos(v_i, v^{t}_j) > cos(v_i, v^{t + 1}_j)\}$. Here, $t \in T$ is the number of intra-class nodes for node $i$, $cos(\cdot)$ is the cosine similarity function. Similarly, we can obtain $L^{inter}_{i} = \{v^{1}_j, ... v^{E}_j| Y_{v^{e}_j} \hlt{\neq Y_i} ; cos(v_i, v^{e}_j) > cos(v_i, v^{e + 1}_j)\}$, where $e \in E$ is the number of inter-class nodes. Finally, we can obtain the ranking list $R_i = \{L^{intra}_{i}[1:K] \parallel L^{inter}_{i}[-K:-1]\}$, which includes top $K$ most similar intra-class and least similar inter-class nodes. The position of each node in $R_i$ determines its true ranking. It is expected that the trained model will identify the correct rank for nodes in ranking lists. The ListNet loss can be formulated as follows:
\begin{equation}
    \hat{\textbf{y}}_i = \textbf{Z}_{gc}[i]^T \cdot \textbf{Z}_{gc}[R_i], 
\end{equation}
\begin{equation}
    % L = -\sum_{i=1}^N \sum_{j=1}^N [Y_i = Y_j] * log(p(Y_i) / p(Y_j))
    \mathcal{L}_{rank} = -\sum^B_{i = 1}(p(\textbf{y}_i)log(p(\hat{\textbf{y}}_i))),
    \label{eq:rank loss}
\end{equation}
where $B$ is the training set size, $p(\cdot)$ is the softmax function, $\hat{\textbf{y}}_i$ is the predicted score list for nodes in ranking list $R_i$, and \hlt{$\textbf{y}_i$ is the true ranking score for nodes in ranking list}.

\paragraph{Graph Complementation} 
\label{par:graph compl}
Combining 
Equation~\ref{eq:group loss} and Equation~\ref{eq:rank loss}, we have the overall loss for training:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{grp} + \mathcal{L}_{rank}.
\end{equation}
Additional homophilic-prone or heterophilic-prone edges are built using the output embedding $\textbf{Z}_{gc}$ from the trained model. For graphs discriminated as homophilic-prone graphs, we find the $K_{heter}$ least similar nodes for each node to find the complemented heterophilic-prone edges. 

In contrast, for graphs discriminated as heterophilic-prone graphs, we find the $K_{homo}$ most similar nodes. The created connections are considered complementary structural information for the graph.


